Towards Effective Rebuttal: Listening Comprehension using Corpus-Wide Claim Mining

Engaging in a live debate requires, among other things, the ability to effectively rebut arguments claimed by your opponent. In particular, this requires identifying these arguments. Here, we suggest doing so by automatically mining claims from a corpus of news articles containing billions of sentences, and searching for them in a given speech. This raises the question of whether such claims indeed correspond to those made in spoken speeches. To this end, we collected a large dataset of $400$ speeches in English discussing $200$ controversial topics, mined claims for each topic, and asked annotators to identify the mined claims mentioned in each speech. Results show that in the vast majority of speeches debaters indeed make use of such claims. In addition, we present several baselines for the automatic detection of mined claims in speeches, forming the basis for future work. All collected data is freely available for research.

==> tablesAndFigures/figure_claim_length_analysis.tex <==
\begin{figure}[h]
\includegraphics[width=8cm]{clen.jpg}
\caption
{The percentage of positive labels for claims of different lengths.}
\label{fig:clen} 
\end{figure}


==> tablesAndFigures/table_ace_claims_vs_idebate_claims.tex <==
\begin{table*}[t]
\begin{center}
\begin{tabular}{|p{0.45\linewidth}|p{0.45\linewidth}|}

\hline \bf \idebate arguments & \bf Additional mined claims \\ \hline
Persuasion is more effective than coercion &
Mandatory voting is absurd in a free society  
\\
\hline
Policing and financing the system is unmanageable & 
Making voting compulsory would be undemocratic 
\\
\hline
There are alternatives that tackle the real causes of voter disengagement &
Enforcement of compulsory voting is likely to be inefficient and expensive 
\\
\hline
\end{tabular}
\end{center}
\caption{Potential arguments for the motion \emph{We should introduce compulsory voting}. 
On the left are arguments taken from \idebate. 
On the right are additional automatically mined claims. 
The first two mined claims are mentioned in at least one recorded speech.
}
\label{tab:ace_claims_vs_idebate_claims} 
\end{table*}
